Searching for GEMS: Characterizing Six Giant Planets around Cool Dwarfs

Transiting giant exoplanets around M-dwarf stars (GEMS) are rare, owing to the low-mass host stars. However, the all-sky coverage of TESS has enabled the detection of an increasingly large number of them to enable statistical surveys like the \textit{Searching for GEMS} survey. As part of this endeavour, we describe the observations of six transiting giant planets, which includes precise mass measurements for two GEMS (K2-419Ab, TOI-6034b) and statistical validation for four systems, which includes validation and mass upper limits for three of them (TOI-5218b, TOI-5616b, TOI-5634Ab), while the fourth one -- TOI-5414b is classified as a `likely planet'. Our observations include radial velocities from the Habitable-zone Planet Finder on the Hobby-Eberly Telescope, and MAROON-X on Gemini-North, along with photometry and high-contrast imaging from multiple ground-based facilities. In addition to TESS photometry, K2-419Ab was also observed and statistically validated as part of the K2 mission in Campaigns 5 and 18, which provides precise orbital and planetary constraints despite the faint host star and long orbital period of $\sim 20.4$ days. With an equilibrium temperature of only 380 K, K2-419Ab is one of the coolest known well-characterized transiting planets. TOI-6034 has a late F-type companion about 40\arcsec~away, making it the first GEMS host star to have an earlier main-sequence binary companion. These confirmations add to the existing small sample of confirmed transiting GEMS.

==> RVs_TOI5176.tex <==
K2-419~A & 2459897.92814 & -931.16 & 153.49 & HPF	 \\ 
K2-419~A & 2459916.87028 & -596.19 & 98.95 & HPF \\ 
K2-419~A & 2459934.00802 & -760.52 & 98.52 & HPF \\ 
K2-419~A & 2459949.96576 & -996.36 & 85.19 & HPF \\ 
K2-419~A & 2459950.77949 & -714.25 & 133.49 & HPF \\ 
K2-419~A & 2459974.71268 & -764.69 & 103.10 & HPF \\ 
K2-419~A & 2459992.66686 & -834.54 & 182.10 & HPF \\ 
K2-419~A & 2460010.80679 & -859.71 & 103.81 & HPF \\ 
K2-419~A & 2460060.66204 & -909.61 & 133.72 & HPF \\ 
K2-419~A & 2460235.08368 & -20.19 & 8.10 & M-X Blue \\ 
K2-419~A & 2460244.11533 & 36.42 & 9.01 & M-X Blue \\ 
K2-419~A & 2460273.05602 & -37.73 & 6.30 & M-X Blue \\ 
K2-419~A & 2460284.10979 & 56.42 & 6.13 & M-X Blue \\ 
K2-419~A & 2460285.14655 & 39.01 & 7.05 & M-X Blue \\ 
K2-419~A & 2460290.15139 & -57.64 & 7.46 & M-X Blue \\ 
K2-419~A & 2460294.03632 & -56.69 & 7.77 & M-X Blue \\ 
K2-419~A & 2460303.11772 & 83.47 & 7.51 & M-X Blue \\ 
K2-419~A & 2460307.06279 & 25.42 & 6.77 & M-X Blue \\ 
K2-419~A & 2460309.02281 & -6.17 & 7.30 & M-X Blue \\ 
K2-419~A & 2460311.08761 & -42.94 & 8.45 & M-X Blue \\ 
K2-419~A & 2460313.13905 & -126.41 & 16.73 & M-X Blue \\ 
K2-419~A & 2460235.08368 & -31.90 & 7.34 & M-X Red \\ 
K2-419~A & 2460244.11533 & 30.41 & 8.40 & M-X Red \\ 
K2-419~A & 2460273.05602 & -45.33 & 5.89 & M-X Red \\ 
K2-419~A & 2460284.10979 & 48.91 & 5.53 & M-X Red \\ 
K2-419~A & 2460285.14655 & 32.14 & 6.43 & M-X Red \\ 
K2-419~A & 2460290.15139 & -47.66 & 6.76 & M-X Red \\ 
K2-419~A & 2460294.03632 & -39.05 & 7.15 & M-X Red \\ 
K2-419~A & 2460303.11772 & 75.69 & 7.17 & M-X Red \\ 
K2-419~A & 2460307.06279 & 11.61 & 6.53 & M-X Red \\ 
K2-419~A & 2460309.02281 & -20.00 & 7.16 & M-X Red \\ 
K2-419~A & 2460311.08706 & -67.78 & 8.13 & M-X Red \\ 
K2-419~A & 2460313.13905 & -84.10 & 16.44 & M-X Red \\ 
%%%
TOI-5218 & 2459833.63890 & -558.74 & 98.92 & HPF \\ 
TOI-5218 & 2459841.60918 & -346.02 & 65.41 & HPF \\ 
TOI-5218 & 2459844.61156 & -437.04 & 81.38 & HPF \\ 
TOI-5218 & 2459846.61287 & -556.06 & 88.74 & HPF \\ 
TOI-5218 & 2459847.61246 & -628.32 & 67.59 & HPF \\ 
%%%
TOI-6034 & 2460143.84965 & 101.60 & 30.23 & HPF \\ 
TOI-6034 & 2460149.83662 & -156.33 & 19.70 & HPF \\ 
TOI-6034 & 2460198.70312 & -151.57 & 25.57 & HPF \\ 
TOI-6034 & 2460210.66716 & 201.62 & 22.39 & HPF \\ 
TOI-6034 & 2460211.66008 & -122.27 & 21.11 & HPF \\ 
TOI-6034 & 2460216.65135 & -127.11 & 18.35 & HPF \\ 
TOI-6034 & 2460219.65046 & -201.28 & 18.66 & HPF \\ 
TOI-6034 & 2460220.64025 & 153.47 & 21.76 & HPF \\ 
TOI-6034 & 2460223.63890 & 129.97 & 27.55 & HPF \\ 
TOI-6034 & 2460224.64075 & -240.80 & 25.09 & HPF \\ 
TOI-6034 & 2460235.59652 & 34.00 & 19.21 & HPF \\ 
%%%
TOI-5414 & 2459857.94350 & 19.41 & 52.07 & HPF \\ 
TOI-5414 & 2459872.90355 & 425.96 & 102.87 & HPF \\ 
TOI-5414 & 2459882.87612 & 143.70 & 54.71 & HPF \\ 
TOI-5414 & 2459890.84374 & 75.86 & 96.28 & HPF \\ 
TOI-5414 & 2459893.85162 & 148.32 & 70.85 & HPF \\ 
TOI-5414 & 2459901.82096 & 90.23 & 81.45 & HPF \\ 
TOI-5414 & 2459906.80485 & -335.17 & 61.05 & HPF \\ 
TOI-5414 & 2459907.80685 & -210.79 & 64.75 & HPF \\ 
TOI-5414 & 2459958.89114 & 108.91 & 61.21 & HPF \\ 
TOI-5414 & 2459965.65462 & 60.77 & 90.91 & HPF \\ 
TOI-5414 & 2459979.83197 & 0.89 & 113.73 & HPF \\ 
TOI-5414 & 2459984.82562 & 110.98 & 58.79 & HPF \\ 
TOI-5414 & 2459986.82689 & 126.77 & 52.28 & HPF \\ 
TOI-5414 & 2460007.76132 & 229.09 & 65.77 & HPF \\ 
TOI-5414 & 2460008.75931 & 89.97 & 53.85 & HPF \\ 
TOI-5414 & 2460009.75749 & 74.73 & 74.43 & HPF \\ 
TOI-5414 & 2460010.75608 & 59.13 & 47.54 & HPF \\ 
TOI-5414 & 2460211.96957 & 191.13 & 62.95 & HPF \\ 
TOI-5414 & 2460312.91890 & 354.30 & 55.61 & HPF \\ 
TOI-5414 & 2460326.88871 & 153.42 & 70.61 & HPF \\ 
TOI-5414 & 2460345.60842 & 191.61 & 73.82 & HPF \\ 
TOI-5414 & 2460364.77799 & 250.52 & 58.29 & HPF \\ 
TOI-5414 & 2460365.79274 & -239.21 & 72.39 & HPF \\ 
TOI-5414 & 2460396.69937 & 317.28 & 58.08 & HPF \\ 
%%%
TOI-5616 & 2459912.01303 & -92.78 & 99.28 & HPF \\ 
TOI-5616 & 2459955.89181 & -268.62 & 80.15 & HPF \\ 
TOI-5616 & 2459957.88893 & -506.11 & 64.95 & HPF \\ 
TOI-5616 & 2459964.86663 & 109.12 & 96.90 & HPF \\ 
TOI-5616 & 2459974.84339 & -232.50 & 86.86 & HPF \\ 
TOI-5616 & 2459980.82857 & -36.46 & 60.25 & HPF \\ 
TOI-5616 & 2460008.96422 & -22.84 & 87.21 & HPF \\ 
TOI-5616 & 2460010.96018 & -170.20 & 55.82 & HPF \\ 
TOI-5616 & 2460064.80724 & -122.47 & 51.47 & HPF \\ 
TOI-5616 & 2460070.78944 & -273.73 & 67.42 & HPF \\ 
TOI-5616 & 2460419.62255 & 67.05 & 63.29 & HPF \\ 
TOI-5616 & 2460423.81855 & -188.43 & 59.72 & HPF \\ 
%%%
TOI-5634 A & 2459923.95858 & -500.11 & 181.52 & HPF \\ 
TOI-5634 A & 2459957.86276 & -128.40 & 173.64 & HPF \\ 
TOI-5634 A & 2459974.81741 & -324.65 & 238.46 & HPF \\ 
TOI-5634 A & 2459978.81112 & -230.77 & 215.94 & HPF \\ 
TOI-5634 A & 2460042.83973 & -953.54 & 356.52 & HPF \\ 
TOI-5634 A & 2460064.78149 & -636.45 & 195.64 & HPF \\ 
TOI-5634 A & 2460070.76247 & -446.02 & 177.19 & HPF \\ 


